Getting into the Flow: Towards Better Type Error Messages for Constraint-Based Type Inference

Creating good type error messages for constraint-based type inference systems is difficult. Typical type error messages reflect implementation details of the underlying constraint-solving algorithms rather than the specific factors leading to type mismatches. We propose using subtyping constraints that capture data flow to classify and explain type errors. Our algorithm explains type errors as faulty data flows, which programmers are already used to reasoning about, and illustrates these data flows as sequences of relevant program locations. We show that our ideas and algorithm are not limited to languages with subtyping, as they can be readily integrated with Hindley-Milner type inference. In addition to these core contributions, we present the results of a user study to evaluate the quality of our messages compared to other implementations. While the quantitative evaluation does not show that flow-based messages improve the localization or understanding of the causes of type errors, the qualitative evaluation suggests a real need and demand for flow-based messages.

==> interactive-errors.tex <==
TODO

\lionel{Here we want to explain how nested type provenance flows can explain errors exhaustively}

Some example expanded flow that could be used and explained


\begin{Error}{\system{}}
\begin{lstlisting}[language=error]
╠════[DETAILED CAUSE]════
╟─> Expression of type [1] : __Double__
║  l.17:‹ 	appInfo = Pair "My Application" _B_1.5__›
╟─>─> flowing into Pair's second argument, with type: Pair Str __Double__
║  l.17:‹ 	appInfo = _B_Pair "My Application" 1.5__›
╟─>─> flowing into argument
║  l.20: 	‹**let** test = process _B_appInfo__›
╟─>─> flowing into pattern
║  l.13:‹ 	process (_B_Pair name vers__) =›
╟─> flowing out of Pair's second pattern, with type [1] : __Double__
║  l.13:‹ 	process (Pair name _B_vers__) =›
╟─> flowing into argument
║  l.14:‹ 	  name ++ show_major (parse_version _B_vers__)›
╟─> does not match expected type: __Str__
║  l.9:‹ 	parse_version: _B_Str__ -> Str›
\end{lstlisting}
\end{Error}

A type provenance chain describes the uninterrupted flow of a type
throughout a program,
aggregating such primitive flow links as:
flowing through a type variable;
flowing into or out of type constructor arguments;
and
flowing into or out of function results and parameters.
% 
Between each of these flow links,
we store associated \emph{program locations},
so type provenance chains
can be seen as structured sequences of program locations.

Complete type provenance chains are \emph{scoped},
in the sense that if a type flows into, say,
a type constructor argument,
then it will also flow out of it later in the chain.
% 
Consequently,
they are type-preserving:
the two ends of a complete type provenance chain always represent
locations at the same type.
% 
As an example, consider the following program:

\begin{lstlisting}
let f p =
  let foo x = Some (x + 1)
  in let bar (Pair x y) = Pair (foo x) (foo y)
  in bar p
in f (Pair 2 3)
\end{lstlisting}

\noi
% We have annotated the different 
% The different flow 
There is a complete type provenance chain which starts at the binding of parameter @p@,
flows into the argument in the call to function @bar@,
into the pattern matched by the definition of @bar@, and stops there.
% 
And there is another complete type provenance chain which \emph{encompasses} that chain;
it starts at the integer literal @2@
of type @Int@,
flows into the first argument of @Pair 2 3@,
thereby temporarily changing its type to @Pair Int Int@,
flows into @p@, then @bar@'s argument, and @bar@'s pattern, as before,
then flows out of the @Pair@ pattern's first sub-pattern @x@,
recovering its initial type @Int@,
and finally flowing into the argument in the first call to function @foo@.

\TODO{add visualization of this paragraph with arrows}


Below is the type full provenance trace provided by our type checker
(\ie what a user would observe if they were to interactively unroll \emph{all} nested flows)
for the type provenance chain mentioned above.

\begin{Error}{\system{}}
\begin{lstlisting}
╟─> Expression of type [1] :  $$__Int__
║  l.7: 	f (Pair __2__ 3)
╟─>─> flowing into Pair's first argument, with type [2] :  Pair $$__Int__ Int
║  l.7: 	f __(Pair 2 3)__
╟─>─>─> flowing into parameter of this function, of type:  Pair $$__Int__ Int -> (?)
║  l.7: 	__f__ (Pair 2 3)
╟─>─>─> flowing from
║  l.3: 	let __f__ p =
╟─>─>─> flowing from
║  l.3: 	let f __p = ...__
╟─>─> of inferred parameter type [2] :  Pair $$__Int__ Int
║  l.3: 	let f __p__ =
╟─>─> flowing into
║  l.6: 	  bar __p__
╟─>─>─> flowing into parameter of this function, of type:  Pair $$__Int__ Int -> (?)
║  l.6: 	  $$__bar__ p
╟─>─>─> flowing from
║  l.5: 	  let __bar__ (Pair x y) = Pair (foo x) (foo y)
╟─>─>─> flowing from
║  l.5: 	  let bar __(Pair x y) = Pair (foo x) (foo y)__
╟─>─> of inferred parameter type [2] :  Pair $$__Int__ Int
║  l.5: 	  let bar (__Pair x y__) = Pair (foo x) (foo y)
╟── flowing out of Pair's first pattern, with type [1] :  $$__Int__
║  l.5: 	  let bar (Pair __x__ y) = Pair (foo x) (foo y)
╟── flowing into
║  l.5: 	  let bar (Pair x y) = Pair (foo __x__) (foo y)
╟─>─> which is a parameter to this function, of inferred type:  $$__Int__ -> (?)
║  l.5: 	  let bar (Pair x y) = Pair (__foo__ x) (foo y)
╟─>─> flowing from
║  l.4: 	  let __foo__ x = Some (x + 1)
╟─>─> flowing from
║  l.4: 	  let foo __x = Some (x + 1)__
╟─> of inferred parameter type [1] :  $$__Int__
║  l.4: 	  let foo __x__ = Some (x + 1)
╟─> flowing into
║  l.4: 	  let foo x = Some (__x__ + 1)
╟─> flowing into expected type: $$__Int__
║  [predef.ml]
║  l.129: 	(+): $$__Int__ -> Int -> Int
\end{lstlisting}
\end{Error}

\noi
% However,
As one can see above,
these traces can become quite long and cumbersome,
especially when lots of abstractions and higher-order functions are used.
Therefore, tracing is \emph{not} a good solution for reporting type error messages to users
most of the time,
and this is why we only provide traces if the \emph{verbose} mode of our type checker is set.





==> mainidea.tex <==
\subsection{Type Mismatch Errors}

Our type inference approach relies on algebraic subtyping
instead of the classical unification-based system.
A direct consequence of this is that we distinguish
two kinds of ML type mismatch errors
which are usually conflated into a single ``unification error'' concept:
\begin{itemize}
  \setlength\itemsep{.4em}
  \item \textbf{\emph{Type collision errors}}
    happen when an actual type ``runs into''
    an incompatible expected type,
    meaning that a term is used in a place
    where a different type is required.
    For example, the term `@not 1@' contains a type collision error
    --- since @1@, of type @Int@, cannot be used as a @Bool@.
    Executing such ill-typed program
    would result in type mismatch errors at runtime
    (\ie non-value terms getting stuck and not reducing further).
  \item \textbf{\emph{Type confluence errors}}
    happen when two incompatible types happen to flow together
    into the same type position,
    for example on either branches of a conditional expression
    such as @if c then True else 1@.
    These errors are \emph{not} actually sources of potential
    runtime errors, and only occur because the ML type system lacks
    a way of representing the union of two distinct types,
    as it does no support subtyping.
\end{itemize}
Algebraic subtyping algorithms like MLsub
will normally \emph{not} report type confluence errors, %by default,
as these are not considered errors in this typing discipline.
However, if desired, it is easy to create an additional phase that runs after
algebraic subtype inference and tries to unify confluent types,
in order to regain %parity
similarity with traditional ML type systems (see \Sec{sec:type-confluence-errors}).
% \TODO{section ... shows how}
In our approach,
type confluence errors will thus be detected in this later phase,
and the approach used to report them will therefore be slightly different.
Nevertheless,
\TODOlater{
we will show \TODO{in ...} that}
the same type provenance infrastructure can be used to report user-friendly
type confluence errors,
as shown in \Sec{sec:type-confluence-errors}.

The distinction between these two kinds of type mismatch errors,
invisible in traditional algorithms but
exposed by algebraic subtyping,
may seem like a technicality,
but it is in fact absolutely crucial.
The amalgamation of type collision and type confluence mismatches by
traditional unification-based system is
one of the reasons that
they typically encounter problems
with the internal ordering of their constraint solving
leading to unstable error message quality.

These two types of errors are special cases for the generalized type error flow
we show below. Type-0 error is the collision error case, where a single type
flow leads to the error. Type-1 error is a confluence error case where two flows
of incompatible types emanate or terminate from the same type location. Type-N
errors generalize this to errors involving N number of flows.

\begin{figure}[H]
  %%
  %% Type 0 Errors
  %%
  \begin{subfigure}{\textwidth}
    \centering
    \begin{minipage}{0.4\textwidth}
      \lstinputlisting{exampleprogs/prog1.txt}
    \end{minipage}
    \hspace{1cm}
    \begin{minipage}{0.4\textwidth}
      \begin{tikzpicture}
        \node (A) at (0,0) {$\mathtt{Int}$};
        \node (B) at (2,0) {$\alpha_x$};
        \node (C) at (4,0) {$\mathtt{Bool}$};
        \draw[->] (A) -- (B);
        \draw[->] (B) -- (C);
      \end{tikzpicture}
    \end{minipage}
    \caption{Program with Type-0 error.}
  \end{subfigure}
  %%
  %% Type 1 Errors
  %%
  \begin{subfigure}{\textwidth}
    \centering
    \begin{minipage}{0.4\textwidth}
      \lstinputlisting{exampleprogs/prog2.txt}
    \end{minipage}
    \hspace{1cm}
    \begin{minipage}{0.4\textwidth}
      \begin{tikzpicture}
        \node (A) at (0,0.5) {$\mathtt{Int}$};
        \node (B) at (0,-0.5) {$\mathtt{String}$};
        \node (C) at (2,0) {$\alpha_{ret}$};
        \draw[->] (A) -- (C);
        \draw[->] (B) -- (C);
      \end{tikzpicture}
    \end{minipage}

    \begin{minipage}{0.4\textwidth}
      \lstinputlisting{exampleprogs/prog3.txt}
    \end{minipage}
    \hspace{1cm}
    \begin{minipage}{0.4\textwidth}
      \begin{tikzpicture}
        \node (A) at (0,0) {$\alpha_x$};
        \node (B) at (2,0.5) {$\mathtt{Int}$};
        \node (C) at (2,-0.5) {$\mathtt{Bool}$};
        \draw[->] (A) -- (B);
        \draw[->] (A) -- (C);
      \end{tikzpicture}
    \end{minipage}
    \caption{Two programs with different Type-1 errors.}
  \end{subfigure}
  %%
  %% Type 2 Errors
  %%
  \begin{subfigure}{\textwidth}
    \centering
    \begin{minipage}{0.4\textwidth}
      \lstinputlisting{exampleprogs/prog4.txt}
    \end{minipage}
    \hspace{1cm}
    \begin{minipage}{0.4\textwidth}
      \begin{tikzpicture}
        \node (A) at (0,-0.5) {$\alpha_x$};
        \node (B) at (0,-1.5) {$\mathtt{Int}$};
        \node (C) at (2,0) {$\mathtt{Bool}$};
        \node (D) at (2,-1) {$\beta_{ret}$};
        \draw[->] (A) -- (C);
        \draw[->] (A) -- (D);
        \draw[->] (B) -- (D);
      \end{tikzpicture}
    \end{minipage}
    \caption{Program with Type-2 error.}
  \end{subfigure}
  \caption{Examples of faulty programs and their corresponding constraint graphs.}
  \end{figure}

